Second-Order Semantic Dependency Parsing with End-to-End Neural Networks

Semantic dependency parsing aims to identify semantic relationships between words in a sentence that form a graph. In this paper, we propose a second-order semantic dependency parser, which takes into consideration not only individual dependency edges but also interactions between pairs of edges. We show that second-order parsing can be approximated using mean field (MF) variational inference or loopy belief propagation (LBP). We can unfold both algorithms as recurrent layers of a neural network and therefore can train the parser in an end-to-end manner. Our experiments show that our approach achieves state-of-the-art performance.

==> graphs/q_value.tex <==
% \documentclass[./messages.tex]{subfiles}
% \documentclass[./test.tex]{subfiles}
%#41017051




%==========================================
%#41105137
% \begin{filecontents*}{qa.txt}
% 94.8 11.0 59.1 2.3
% 21.8 43.6 72.6 2.9
% 3.0 0.4 4.6 0.2
% 5.4 33.5 17.5 24.6
% 21.5 15.6 63.5 0.1

% \end{filecontents*}
% \begin{filecontents*}{qb.txt}
% 76.5 0.0 1.1 0.0
% 0.4 57.8 74.8 0.2
% 0.1 0.1 0.8 0.0
% 0.3 58.4 0.4 22.6
% 1.4 1.5 45.2 0.0

% \end{filecontents*}
% \begin{filecontents*}{qc.txt}
% 98.6 0.2 4.1 0.1
% 0.3 46.1 89.9 0.1
% 0.2 0.1 1.3 0.0
% 0.4 46.1 0.6 8.2
% 5.6 6.5 81.2 0.0

% \end{filecontents*}
% \begin{filecontents*}{qd.txt}
% 98.4 0.1 1.2 0.1
% 0.1 54.2 91.3 0.1
% 0.1 0.2 1.6 0.0
% 0.4 72.3 0.5 12.5
% 0.7 1.2 73.5 0.0
% \end{filecontents*}
%#41105137
% \begin{filecontents*}{qa.txt}
% 0.0 94.8 11.0 59.1 2.3
% 0.0 21.8 43.6 72.6 2.9
% 0.0 3.0 0.4 4.6 0.2
% 0.0 5.4 33.5 17.5 24.6
% 0.0 21.5 15.6 63.5 0.1

% \end{filecontents*}
% \begin{filecontents*}{qb.txt}
% 0.0 76.5 0.0 1.1 0.0
% 0.0 0.4 57.8 74.8 0.2
% 0.0 0.1 0.1 0.8 0.0
% 0.0 0.3 58.4 0.4 22.6
% 0.0 1.4 1.5 45.2 0.0

% \end{filecontents*}
% \begin{filecontents*}{qc.txt}
% 0.0 98.6 0.2 4.1 0.1
% 0.0 0.3 46.1 89.9 0.1
% 0.0 0.2 0.1 1.3 0.0
% 0.0 0.4 46.1 0.6 8.2
% 0.0 5.6 6.5 81.2 0.0

% \end{filecontents*}
% \begin{filecontents*}{qd.txt}
% 0.0 98.4 0.1 1.2 0.1
% 0.0 0.1 54.2 91.3 0.1
% 0.0 0.1 0.2 1.6 0.0
% 0.0 0.4 72.3 0.5 12.5
% 0.0 0.7 1.2 73.5 0.0

% \end{filecontents*}

% \begin{filecontents*}{qa.txt}
% 0.0 6.5 25.2 0.9 50.8
% 0.0 0.0 0.0 0.0 0.0
% 0.0 14.6 0.6 26.7 71.9
% 0.0 0.0 0.0 0.0 0.0
% 0.0 3.1 1.7 26.9 1.4

% \end{filecontents*}
% \begin{filecontents*}{qb.txt}
% 0.0 1.6 38.3 0.1 6.4
% 0.0 0.0 0.0 0.0 0.0
% 0.0 26.5 0.0 30.6 49.3
% 0.0 0.0 0.0 0.0 0.0
% 0.0 2.2 0.4 13.6 0.0

% \end{filecontents*}
% \begin{filecontents*}{qc.txt}
% 0.0 0.7 70.1 0.1 7.2
% 0.0 0.0 0.0 0.0 0.0
% 0.0 32.4 0.0 47.2 89.5
% 0.0 0.0 0.0 0.0 0.0
% 0.0 0.7 0.1 5.8 0.1

% \end{filecontents*}
% \begin{filecontents*}{qd.txt}
% 0.0 0.2 89.9 0.0 0.6
% 0.0 0.0 0.0 0.0 0.0
% 0.0 59.0 0.0 83.5 95.9
% 0.0 0.0 0.0 0.0 0.0
% 0.0 0.4 0.0 2.0 0.0

% \end{filecontents*}


% \end{comment}
